Sliding-Mode Control Strategies for PMSM: Benchmarking and Comparative Simulation Study

Permanent Magnet Synchronous Motors (PMSMs) are widely employed in high-performance drive systems owing to their high efficiency and power density. However, nonlinear dynamics, parameter uncertainties, and load disturbances complicate their control. Sliding-Mode Control (SMC) offers strong robustness but exists in numerous variants with unstandardized evaluation criteria. This paper presents a unified simulation benchmark and comparative analysis of six representative SMC techniques for PMSM speed regulation: conventional, integral, terminal, fractional-order, adaptive, and super-twisting. A standardized PMSM model, disturbance profile, and tuning protocol are adopted to ensure fair comparison across all methods. Performance is assessed through time-domain responses, integral error indices (ISE, IAE, ITSE, ITAE), and control-effort profiles, while also examining computational complexity and implementation feasibility. Results demonstrate that adaptive and higher-order SMCs, particularly the super-twisting and adaptive variants, achieve the most balanced trade-off between robustness, smoothness, and computational cost. The study provides a reproducible benchmarking framework, parameter-selection guidelines, and practical insights for designing efficient, low-chatter SMC-based PMSM drives suitable for real-time embedded implementation.

==> ResearchPyramidFigure.tex <==
% ===================== Research Pyramid Figure ======================
\begin{figure*}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[>=stealth, node distance=2.4cm, every node/.style={align=center}]

% helper macro: draw a colored trapezoid layer
% args: y, width_bottom, width_top, height, fillcolor, title, bullets
\newcommand{\layer}[7]{
  \def\y{#1}\def\wb{#2}\def\wt{#3}\def\h{#4}\def\col{#5}
  \def\titletext{#6}\def\bullets{#7}
  % coordinates (centered at x=0)
    \path (-\wb/2,\y) coordinate (L\y)  (\wb/2,\y) coordinate (R\y);
    \path (-\wt/2,\y+\h) coordinate (Lt\y)  (\wt/2,\y+\h) coordinate (Rt\y);
  
  % shape
  \filldraw[draw=black, thick, fill=\col] (L\y) -- (R\y) -- (Rt\y) -- (Lt\y) -- cycle;
  % text box
  \node[align=center, text width=\wt-0.6cm] at (0,\y+\h/2)
    {\textbf{\titletext}\\[2pt]\bullets};
}

% ----- layers (bottom -> top) -----
\layer{0}{12}{10}{2.1}{gray!15}
  {Foundations: Classical/Terminal SMC}
  {Robust invariance; high/medium chattering\\
   Simple DSP deployment; baseline for benchmarks}

\layer{2.3}{10}{8}{2.1}{blue!12}
  {Observer- and Adaptive-Enhanced SMC}
  {ESO/DOB/SMO integration; online gain tuning\\
   Better disturbance rejection with smooth actuation}

\layer{4.6}{8}{6}{2.1}{green!12}
  {Fractional-Order \& Hybrid Designs}
  {Memory effects for shaping transients; fractional–adaptive blends\\
   Careful discretization to avoid bias/instability}

\layer{6.9}{6}{4.8}{2.1}{orange!12}
  {Intelligent Tuning}
  {RL/NN/Fuzzy/Meta-heuristics for auto-tuning\\
   Data efficiency, stability guarantees, and safety filters}

\layer{9.2}{4.8}{3.6}{2.1}{yellow!25}
  {Experimental Validation}
  {Real-time DSP/FPGA, EMI/thermal constraints\\
   HIL, energy use, switching stress, reliability}

\layer{11.5}{3.6}{2.8}{2.1}{purple!15}
  {Standardization \& Deployment}
  {Open benchmarks, reproducible code/models\\
   Application-specific KPIs \& certification}

% title arrow
\draw[->,very thick] (0,-0.7) -- (0,14.0) node[above,font=\bfseries] {Future Work Trajectory};

% side labels
\node[rotate=90] at (-7.2,6.3) {\textbf{Complexity / Effort} $\uparrow$};
\node[rotate=90] at ( 7.2,6.3) {\textbf{Impact / Readiness} $\uparrow$};

\end{tikzpicture}}
\caption{Vertical research pyramid for PMSM SMC: progressing from foundational designs (base) to observer/adaptive enhancement, fractional and hybrid methods, intelligent tuning, experimental validation, and finally standardization and deployment (apex).}
\label{fig:research_pyramid_smc}
\end{figure*}
% ================== End Research Pyramid Figure =====================

